Optimal high-precision shadow estimation

We give the first tight sample complexity bounds for shadow tomography and classical shadows in the regime where the target error is below some sufficiently small inverse polynomial in the dimension of the Hilbert space. Formally we give a protocol that, given any $m\in\mathbb{N}$ and $\epsilon \le O(d^{-12})$, measures $O(\log(m)/\epsilon^2)$ copies of an unknown mixed state $\rho\in\mathbb{C}^{d\times d}$ and outputs a classical description of $\rho$ which can then be used to estimate any collection of $m$ observables to within additive accuracy $\epsilon$. Previously, even for the simpler task of shadow tomography -- where the $m$ observables are known in advance -- the best known rates either scaled benignly but suboptimally in all of $m, d, \epsilon$, or scaled optimally in $\epsilon, m$ but had additional polynomial factors in $d$ for general observables. Intriguingly, we also show via dimensionality reduction, that we can rescale $\epsilon$ and $d$ to reduce to the regime where $\epsilon \le O(d^{-1/2})$. Our algorithm draws upon representation-theoretic tools recently developed in the context of full state tomography.

==> tech-overview.tex <==
\section{Technical overview}
\label{sec:overview}

\subsection{Basic Setup}

Throughout, let $\rho$ denote a mixed state.
We recall that a mixed state is described by its density matrix, a PSD Hermitian matrix in $\C^{d\times d}$ with trace $1$.  We use $I_d$ to denote the $d \times d$ identity matrix.

\paragraph{Measurements.}  
%\sitan{we can probably move this part to the prelims} 
We now define the standard measurement formalism, which is the way algorithms are allowed to interact with a quantum state $\rho$.
\begin{definition}[Positive operator valued measurement (POVM), see e.g.~\cite{nielsen2002quantum}]
A positive operator valued measurement $\cM$ in $\C^{d \times d}$ is a collection of PSD matrices $\cM = \{M_z\}_{z \in \cZ}$ satisfying $\sum_z M_z = I_d$.  When a state $\rho$ is measured using $\cM$, we get a draw from a classical distribution over $\cZ$, where we observe $z$ with probability $\tr (\rho M_z)$.
Afterwards, the quantum state is destroyed.
\end{definition}

\noindent 

\paragraph{$t$-Entangled Measurements}
% Next, we formally define what we mean by an algorithm that uses incoherent measurements.
An algorithm that uses $t$-entangled measurements and $n$ total copies of $\rho$ operates as follows: it is given $m = n/t$ copies of $\rho^{\otimes t}$.  It then iteratively measures the $i$-th copy of $\rho^{\otimes t}$ (for $i = 1,2, \dots , m$) using a POVM  in $\C^{d^t \times d^t}$ which could depend on the results of previous measurements, records the outcome, and then repeats this process on the $(i + 1)$-th copy.  After having performed all $m$ measurements, it must output an estimate of $\rho$ based on the (classical) sequence of outcomes it has received.


\begin{remark}
Note that limiting the batch size to exactly $t$ is not actually a limitation because we can simulate an algorithm that adaptively chooses batch sizes of at most $t$ with an algorithm that uses batch sizes of exactly $t$ up to at most a factor of $2$ in the total copy complexity.  This is because we can simply combine batches whenever their total size is at most $t$.   
\end{remark}

\subsection{Key Technical Tools}
Now we introduce some of the key technical tools used in both the upper and lower bound.


\subsubsection{Power Series Approximation}\label{sec:power-series}

It will be instructive to first consider the case where $\rho$ is close to the maximally mixed state.  Write $\rho = I_d/d + E$ for some $E \in \C^{d \times d}$.  Observe that when $E$ is small, we can approximate
\begin{equation}\label{eq:intro-powerseries}
\rho^{\otimes t} \sim (I_d/d)^{\otimes t} + \sum_{sym} E \otimes (I_d/d)^{\otimes t-1} \,.
\end{equation}
Let the LHS of the above be $X$ and the RHS be $X'$.  In general $X'$ will be significantly easier to work with than $X$ when analyzing various measurements so when the above approximation is good, we can work with $X'$ in place of $X$.  Now consider a POVM, say $\{\omega_z zz^\dagger \}_{z \in \calZ}$ in $\C^{d^t \times d^t }$ where $z$ are unit vectors and $\omega_z$ are nonnegative weights (WLOG it suffices to consider rank-$1$ POVMs, see e.g. \cite{chen2022exponential, chen2022tight, chen2023does}).  Now consider constructing an estimator $f(z): \C^{d^t} \rightarrow \C^{d \times d}$ that is supposed to estimate $E$.  The expectation after measuring $X'$ is %\footnote{$X'$ may not technically be a state but all of the quantities we work with will still be well-defined} 
\begin{equation}\label{eq:intro-estimator}
\E[ f(z)] = \int f(z) \langle X' ,  \omega_z zz^\dagger \rangle dz \,.
\end{equation}
The above is a linear function in the entries of $E$ since $X'$ is linear in $E$, and as long as $f(z)$ is chosen appropriately, it will be a linear function of the matrix $E$.  We can write it as $Y  + cE$ for some constant matrix $Y$ (which will be a multiple of $I_d$ by symmetry) and constant $c$.  Now, we have an estimator, given by $f(z)$, whose mean is $cE$ (as we can simply subtract off $Y$) and whose variance is equal to the average of $\norm{f(z)}_F^2$.  Let
\[
\theta = \int \omega_z \norm{f(z)}_F^2 dz \,. 
\]
The quantity $\theta$ controls the variance of our estimator.  Technically $\theta$ is the average of $\norm{f(z)}_F^2$ when measuring the maximally mixed state but when $E$ is small, it is the same up to constant factors as the average of $\norm{f(z)}_F^2$ when measuring $X'$.  Thus, the sample complexity that we need to estimate $E$ to accuracy $\eps$ in Frobenius norm is $O( \theta /(c^2\eps^2))$ \--- in particular it scales linearly in the variance $\theta$ and inverse quadratically with the ``signal" $c$ in the estimator.

%\jerry{maybe this paragraph should be slightly rewritten}


Now it suffices to maximize the ratio $c^2/\theta$.  We can express $\langle X', \omega_z z z^\dagger \rangle = \frac{\omega_z}{d^t} + \frac{\omega_z}{d^{t-1}}\langle E,  G_1(z) \rangle$ where the matrix $G_1(z)$ is constructed as follows (see Section~\ref{sec:lower-bound-tools} for more details): 
\begin{itemize}
    \item Rearrange $z$ into a $\underbrace{d \times \dots \times d}_t$ tensor 
    \item Let $F_1(z), \dots , F_t(z)$ be the $t$ different ways to unfold this tensor into a $d \times d^{t-1}$ matrix by flattening all but one of the modes. 
    \item Set $G_1(z) = F_1(z)F_1(z)^\dagger + \dots + F_t(z) F_t(z)^\dagger $
\end{itemize}

\noindent Roughly, we can think of maximizing $c$ as the same as maximizing $\E[\langle f(z), E \rangle ]$.  We can write
\[
\E[\langle E , f(z) \rangle] = \frac{1}{d^{t-1}} \int \omega_z \langle E, f(z) \rangle \langle E, G_1(z) \rangle dz \,.
\]
The above is a linear function in $f(z)$ and roughly, we are trying to maximize it subject to a norm constraint on $\norm{f(z)}_F^2$ so a natural choice for $f(z)$ (that turns out to be optimal) is $f(z) = G_1(z)$.  In this case, we can compute that both $c$ and $\theta$ scale with $\int \omega_z \norm{G_1(z)}_F^2 dz$ and thus the quotient $c^2/\theta$ scales linearly as well.  We get that
\[
\frac{c^2}{\theta} \sim  \frac{1}{d^2} \int \omega_z \norm{G_1(z)}_F^2 dz \,.
\]
In other words, it suffices to understand the average Frobenius norm of the unfolded matrix $G_1(z)$.
%\allen{Is this any better?}

\subsubsection{Bounding the Unfolded Matrix}\label{sec:unfolded-matrix}

The key insight in understanding $\norm{G_1(z)}_F^2$ is that it is actually related to the projection of $z$ onto the different Schur subspaces.  We prove in Lemma~\ref{lem:skewness-bound} that 
\begin{equation}\label{eq:key-eq-intro}
\norm{G_1(z)}_F^2 \leq \norm{z}^2 \sum_{\lambda \vdash t} \norm{\Pi_{\lambda} z}^2 ( \lambda_1^2 + \dots + \lambda_d^2) 
\end{equation}
where the sum is over all partitions $\lambda$ of $t$ and $\Pi_{\lambda}$ denotes the projection onto the $\lambda$-Schur subspace of $\C^{d^t}$ (see Section~\ref{sec:rep-theory} for formal definitions).  The point is that the distribution over partitions $\lambda \vdash t$ induced by the projections $\Pi_{\lambda}$ is exactly the well-studied Schur-Weyl distribution.  Since $\{ \omega_z zz^\dagger\}$ need to form a POVM, the average of $\norm{G_1(z)}_F^2$ is roughly determined by the value of $\lambda_1^2 + \dots + \lambda_d^2$ for a ``typical" partition drawn from the Schur-Weyl distribution.   We prove that this typical value is exactly $\Theta(t^{1.5})$ when $t \leq d^2$ (see Claim~\ref{claim:typical-young-tableaux1} and Claim~\ref{claim:typical-young-tableaux2}).  For our learning algorithm, we show that Keyl's POVM actually achieves $\norm{G_1(z)}_F^2 \sim t^{1.5}$ for most $z$ in the POVM.  For our lower bound, we formalize the intuition that the quantity $\norm{G_1(z)}_F^2$ precisely controls the ``information" gained by the learner after each measurement.


\subsection{Learning Algorithm}

Section~\ref{sec:power-series} and Section~\ref{sec:unfolded-matrix} already give the blueprint for the learning algorithm when $\rho$ is close to maximally mixed.  In particular, we have a POVM (namely Keyl's POVM) given by $\{\omega_z zz^\dagger \}_{z \in \calZ}$ in $\C^{d^t \times d^t}$ such that $\norm{G_1(z)}_F^2 \sim t^{1.5}$ for most $z$ and thus using the estimator $f(z) = G_1(z)$ in \eqref{eq:intro-estimator}, we can use $d^2/(t^{1.5} \eps^2)$ batches and compute $\wh{\rho}$ such that $\norm{\wh{\rho} - \rho}_F \leq \eps$.   


\subsubsection{Rotational Invariance}

We first note that naively, the approximation \eqref{eq:intro-powerseries} seems to require $t \ll 1/(d\norm{E})$.  However, we can exploit the symmetries in Keyl's POVM to deduce that the approximation holds for a much larger range of $t$.  We show that the approximation holds up to $t \sim (1/\norm{E}_F)^c$ for some small constant $c$.  In particular, we obtain nontrivial guarantees even when $\norm{E}  \gg 1/d$ (this is why Theorem~\ref{thm:upper-informal} works up to $t \sim (d/\eps)^c$ instead of just $t \sim (1/\eps)^c$).   The key point is that Keyl's POVM is copywise rotationally invariant, meaning that for a unitary $U \in \C^{d \times d}$, applying $U^{\otimes t} zz^\dagger (U^\dagger)^{\otimes t}$ to all of the elements of the POVM results in the same POVM.  The key lemma is Lemma~\ref{lem:random-rotations}, which shows that for any matrix $E$ and unit vector $v$,
\begin{equation}\label{eq:intro-rotation}
{d^t} \left\lvert \E_{U}[\langle (U E U^{\dagger})^{\otimes t}, vv^\dagger \rangle  ] \right\rvert \leq (4t)^{4t} \norm{E}_F^t
\end{equation}
where the expectation is over Haar random unitaries $U$.  In particular, due to the random rotation on the LHS, the RHS scales with $\norm{E}_F$ instead of $d\norm{E}$.  We can use \eqref{eq:intro-rotation} to bound the contribution of the terms of order-$2$ and higher in the expansion $\rho^{\otimes t} = (I_d/d + E)^{\otimes t}$.  Roughly the point is that for constant $k$, there are $\binom{t}{k}$ terms of order-$k$ and they are bounded by  $\norm{E}_F^k$, so as long as $t \sim \norm{E}_F^c$ for some small constant $c$, the error terms in the truncation in \eqref{eq:intro-powerseries} decay geometrically.     



\subsubsection{A Multi-stage Approach via Quantum Splitting}

The algorithm we sketched so far only works when $\rho$ is close to $I_d/d$.  
It remains to show how to make it work for general states.
We do so in two steps.
First, we can bootstrap this to learn $\rho$ whenever $\norm{\rho} \leq 2/d$.
This is because we can first obtain a rough estimate $\wh{\rho}$ and then simulate access to the state $\frac{\rho + (2I_d/d - \wh{\rho})}{2}$.  This state is close to maximally mixed so we can obtain a finer estimate of $\rho - \wh{\rho}$ which allows us to refine our estimate of $\rho$.  Note that the same argument works whenever   $\norm{\rho} \leq C/d$ for some constant $C$.

Next, when $\norm{\rho}$ is large, we rely on a splitting procedure that transforms a state $\rho$ into a state $\Split(\rho)$ such that 
\begin{itemize}
\item $\norm{\Split(\rho)} \leq C/d$ for some constant $C$
\item We can simulate measurement access to copies of $\Split(\rho)$ given measurement access to copies of $\rho$
\end{itemize}  
The way the splitting procedure works is as follows: we first (approximately) diagonalize $\rho$.  Let its eigenvalues be $\alpha_1, \dots , \alpha_d$.  For each $j$, let $b_j$ be the smallest nonnegative integer such that $\alpha_j \leq 2^{b_j}/d$.  Then $\Split(\rho)$ is a $k \times k$ matrix where $k = 2^{b_1} + \dots + 2^{b_d}$ (note that $k \leq 4d$).  For each $j$, we split the $j$th row and column of $\rho$ into $2^{b_j}$ rows and columns and divide the entries evenly between these rows and columns (see Definition~\ref{def:split}).  Note that we lose a factor of $2^{\max(b_1, \dots , b_d)/2}$ in our recovery guarantee due to the splitting procedure.  Thus, we incorporate a multi-scale approach where we consider projecting out eigenvalues and splitting  at different scales.  Due to this, our final recovery guarantee for learning general states is in trace norm instead of Frobenius norm. 
 See Section~\ref{sec:embedding} for more details.    


%Say something about accuracy guarantee




\subsection{Lower Bound}

The lower bound follows the likelihood ratio framework of \cite{chen2023does} and the key new ingredient is the upper bound on the average Frobenius norm of $G_1(z)$ in \eqref{eq:key-eq-intro}.  Recall the high level framework in \cite{chen2023does}.  There is some prior distribution on valid quantum states $\rho$.  The unknown state $\rho_0$ is sampled from this distribution.  After making a sequence of measurements and observing outcomes, say $z_1, \dots , z_m$ where $m = n/t$, we have some posterior distribution over states $\rho$ and learning succeeds only when the posterior concentrates around $\rho_0$.  The posterior measure at some alternative hypothesis $\rho$ is 
\begin{equation}
\frac{\mu_{\textsf{post}}(\rho)}{\mu_{\textsf{post}}(\rho_0)} = \prod_{j = 1}^m \frac{z_j^\dagger \rho^{\otimes t} z_j}{z_j^\dagger \rho_0^{\otimes t} z_j} \,.
\end{equation}
Let $\rho$ have $\norm{\rho - \rho_0}_1 \geq C_1\eps$ and $ \norm{\rho - \rho_0} \leq C_2\eps/d$ for some constants $C_1, C_2$.  Then to prove a lower bound, it roughly suffices to show that the above ratio is at least $\exp(-d^2)$ (this is because the volume of the ball of alternative hypotheses is $\exp(d^2)$ times the volume of valid outputs with respect to $\rho_0$).


To lower bound the above ratio, it suffices to show that the update to the ratio in each step is at most $\exp( -\eps^2 t^{1.5}/d )$ on average.  The key lemma that proves this is Lemma~\ref{lem:avg-likelihood-ratio}.  While the full lemma is a bit more complicated and only holds in an average-case sense, for the purposes of this overview, we can think of the lemma as saying that 
\[
\frac{z^\dagger \rho^{\otimes t} z}{z^\dagger \rho_0^{\otimes t} z} \geq \exp\left( -\frac{\norm{G_1(z)}_F^2 \eps^2}{d} \right) \,.
\]  
Now, in Section~\ref{sec:unfolded-matrix}, we argued that for any POVM, $\norm{G_1(z)}_F^2$ can be at most $O(t^{1.5})$ on average so typically, the above ratio will be at least $\exp\left(-\frac{t^{1.5} \eps^2}{d}   \right)$.  Thus, as long as $m \leq d^3/(t^{1.5} \eps^2 )$, which is the same as $n \leq d^3/(\sqrt{t} \eps^2)$, then $\frac{\mu_{\textsf{post}}(\rho)}{\mu_{\textsf{post}}(\rho_0)} \geq \exp(-d^2)$ and this completes the sketch of the lower bound.

